AI-Assisted Scientific Assessment: A Case Study on Climate Change

The emerging paradigm of AI co-scientists focuses on tasks characterized by repeatable verification, where agents explore search spaces in 'guess and check' loops. This paradigm does not extend to problems where repeated evaluation is impossible and ground truth is established by the consensus synthesis of theory and existing evidence. We evaluate a Gemini-based AI environment designed to support collaborative scientific assessment, integrated into a standard scientific workflow. In collaboration with a diverse group of 13 scientists working in the field of climate science, we tested the system on a complex topic: the stability of the Atlantic Meridional Overturning Circulation (AMOC). Our results show that AI can accelerate the scientific workflow. The group produced a comprehensive synthesis of 79 papers through 104 revision cycles in just over 46 person-hours. AI contribution was significant: most AI-generated content was retained in the report. AI also helped maintain logical consistency and presentation quality. However, expert additions were crucial to ensure its acceptability: less than half of the report was produced by AI. Furthermore, substantial oversight was required to expand and elevate the content to rigorous scientific standards.

==> sections/0a-abstract.tex <==
The emerging paradigm of AI co-scientists focuses on tasks characterized by repeatable verification, where agents explore search spaces in 'guess and check' loops. This paradigm does not extend to problems where repeated evaluation is impossible and ground truth is established by the consensus synthesis of theory and existing evidence. We evaluate a Gemini-based AI environment designed to support collaborative scientific assessment, integrated into a standard scientific workflow. In collaboration with a diverse group of 13 scientists working in the field of climate science, we tested the system on a complex topic: the stability of the Atlantic Meridional Overturning Circulation (AMOC).
Our results show that AI can accelerate the scientific workflow. The group produced a comprehensive synthesis of 79 papers through 104 revision cycles in just over 46 person-hours. AI contribution was significant: most AI-generated content was retained in the report. AI also helped maintain logical consistency and presentation quality. However, expert additions were crucial to ensure its acceptability: less than half of the report was produced by AI. Furthermore, substantial oversight was required to expand and elevate the content to rigorous scientific standards.

==> sections/1-Introduction.tex <==
\section{Introduction}
\label{sect:intro}

\begin{figure*}
    \centering
    \includegraphics[width=0.99\linewidth]{images/history_flow_combined_s2_s3_document.pdf}
    \caption{\small The evolution of the AMOC report, visualized as a \emph{history flow}~\citep{Viegas-et-al-2004}, a method introduced to analyze the edit history of Wikipedia articles. We visualize only the main body, excluding references which are section-specific in Phase 2 then unified in Phase 3. Transitions between versions are represented as vertical bands. Edits are attributed via color-coded horizontal bands. The \assistant provided the first version (0). Visually, the process is a somewhat chaotic, rich weaving of AI and human contributions.}
    \label{fig:history-flow-phases12-anonym}
\end{figure*}
The emergence of AI \emph{co-scientists}, agentic systems capable of autonomous hypothesis generation and experimental design, marks a paradigm shift in scientific discovery~\citep{boiko2023autonomous,gottweis2025}. Current co-scientists are self-evaluating, parallelizable pipelines of Large Language Model (LLM) calls  
that search hypothesis spaces at a massive scale to brainstorm and propose candidate ideas for validation in real-world experiments. 

This approach shines in \emph{verification-rich} tasks such as drug discovery~\citep{gottweis2025} or code optimization~\citep{lu2024aiscientist}, where ground truth is accessible via immediate feedback loops in well-structured repeatable experiments. \citet{Knusel2019} characterize these as ``small problems'': the cost of AI hallucination is low because reality provides immediate error correction. In contrast, some high-stakes research questions in fields such as macro-economics, epidemiology and climate science are \emph{verification-poor}: controlled experiments are often impossible, systems are non-stationary \citep{lucas1976econometric}, and truth is an authoritative state of knowledge that is arrived at through scientific consensus construction rather than measurement \citep{cleland2002methodological}.\footnote{Most fields span both verification-rich and verification-poor aspects. Climate science combines verification-rich foundations ($\mathrm{CO}_2$ levels, radiative forcing) and verification-poor complexities (e.g., Earth's tipping points) where model dependence and deep uncertainty require integrative assessment rather than verification.}
Consequently, establishing the state of knowledge requires not just calculation, but \emph{assessment}—weighing reinforcing and diverging evidence against background theory to form a consensus \citep{baumberger2017, oreskes2004scientific}.

Realistically, the deployment of AI in these high-stakes applications is still in its infancy~\citep{Human_AI_DRR}. We argue that trusted full-stack AI co-scientists require the \emph{integration} of them within the collaborative assessment process, to support researchers in formulating, refining, and addressing complex research questions, while operating under direct expert oversight~\citep{wang2019human}.
We present a first empirical evaluation of such an AI \assistant, deeply integrated into a realistic workflow. The \assistant was stress-tested by renowned climate scientists\footnote{Among the authors of this work.} on a complex topic: the stability of the Atlantic Meridional Overturning Circulation (AMOC), a system of ocean currents that transports heat and nutrients across the Atlantic, and contributes to regulating the global climate~\citep{Rahmstorf-Oceanography-2024}. 
Ongoing scientific debate, driven by conflicting evidence from observations, proxy records, and climate models, makes AMOC an especially demanding and informative case study.

We hypothesize that an integrated assistant could enhance the scientific synthesis process by improving: efficiency (accelerating drafting and review), consistency (maintaining a unified voice and evidence assessment), traceability (the ability to easily audit and link conclusions directly to literature, comments, messages and previous versions of the text, adhering to an ``OpenReview principle''), and collaboration (facilitating communication and consensus finding). 
The main findings of our experiment include:
\begin{itemize}[leftmargin=*, topsep=0pt, itemsep=2pt, partopsep=0pt, parsep=0pt]
    \item {\bf A productive hybrid framework}: The \assistant provided a productive environment for the assessment. According to the participating scientists, the final output, an 8,000 words report synthesizing findings from 79 papers, forms a solid basis for a manuscript and assessment outcome that would be suited for scrutiny by scientific peer-review, be it as a journal submission or as part of the preparation process of a scientific assessment report.\footnote{The main report versions are included in the Appendix.}
    \item {\bf High efficiency}: The process demonstrated efficiency and convergence (cf. Figure~\ref{fig:history-flow-phases12-anonym}, Figure~\ref{fig:convergence}). 
    Writing the assessment, through 104 intermediate versions, took the 13 scientists 46 hours, 36 minutes total. Self-reported estimates of perceived efficiency gains range from 3-5x 
    to 17x, depending on the rationale. 
    \item {\bf Significant AI contributions}: 
    The vast majority, more than 90\%, of the AI-generated content was retained, after being checked and accepted by the scientists. At times the content was, however, significantly improved in the final version. AI-generated revisions were utilized 3 times more frequently than manual ones, with AI credited for approximately $25\%$ of the revisions content. 
    \item {\bf Expert human oversight is critical}: While AI content is retained, human intervention is critical for scientific rigor. The scientists contributed $58.4\%$ of the final report's content ($37.2\%$ for the outline). Human edits were essential to elevate the content from a high-quality general summary to a rigorous scientific synthesis and assessment. 
    \item {\bf Challenges}: We occasionally observed well-known limitations of LLMs involving difficulties synthesizing quantitative data, obsequiousness (especially when pushed adversarially), a lack of holistic reasoning (e.g., identifying caveats), and hallucinations (e.g., reconciling reference numbering). Overall, the negative impact of such behaviors was mitigated by extensive human oversight. Notably, this framework may enhance scrutiny by allowing experts to focus on review rather than drafting. We conclude that while the \assistant produces a {solid basis}, {final expert verification} remains essential to reach {peer-review quality}.
\end{itemize}

Overall, AI proved effective at summarizing content and maintaining technical consistency. However, its utility depended on expert guidance. AI currently lacks the deep understanding required for complex topics like AMOC~\citep{messeri2024artificial}, where full comprehension often relies on tacit knowledge held by a few specialists. These limitations likely extend to other complex 'verification-poor' problems. While AI cannot yet replace human scientists, it has significant potential to accelerate their workflows. Moreover, human-AI collaboration creates a feedback loop that can improve the AI's grasp of scientific processes and offers new ways to evaluate its capabilities.


==> sections/1b-relatedliterature.tex <==
\section{Related Work}

The integration of agentic AI into scientific workflows marks a transition from passive data analysis to autonomous knowledge generation \citep{gridach2025agentic, wang2023scientific}. 

The most robust successes of agentic AI have occurred in verification-rich environments—domains where hypotheses can be rigorously tested against a programmatic or physical ground truth. \citet{hartung2025ai} describes this as the shift to "scAInce", exemplified by \citet{romeraparedes2024mathematical} using code execution to verify mathematical proofs, and \citet{boiko2023autonomous, bran2024chemcrow} automating chemical synthesis. \citet{lu2024aiscientist} pushed this paradigm to automate the entire lifecycle with \textit{The AI Scientist}. 
However, despite these advancements, technical quality challenges persist~\citep{beel2025evaluating_arxiv}. 
It is not yet clear how to extend this architecture to domains where truth is a theoretical consensus rather than an experimental outcome.

In climate science, 'ground truth' is complicated by data friction, the difficulty of constructing global truths from heterogeneous observations \citep{edwards2013vast}. While AI has revolutionized \textit{simulation} (e.g., GraphCast \citep{lam2023learning}, NeuralGCM \citep{kochkov2024neural}), these tools function as dynamical emulators, not epistemic assessors, often biasing collective attention toward data-rich operational questions rather than foundational ones \citep{Hao2026}. These models can predict state evolution using low-dimensional embeddings \citep{moore2025automated}, but lack the explanatory capacity to assess complex phenomena. \citet{baumberger2017} warn that empirical fit does not imply adequacy for long-term projection, mirroring \citeauthor{lucas1976econometric}'s critique that statistical models fail when structural conditions change \citep{lucas1976econometric}. Thus, climate AI requires reasoning architectures \citep{202504.2088} beyond token prediction. Ultimately, the scientific assessment problem is not a peculiarity of climate science, but a defining aspect of the scientific method itself.

In the absence of physical verification, AI relies mostly on textual evidence \citep{zheng2023large, asai2024openscholar}. While systems like DeepScholar \citep{patel2025deepscholar} and automated reviews \citep{cao2025automation} show promise, they introduce specific challenges. \citet{messeri2024artificial} warn of an "illusion of understanding", where fluent explanations mask shallow reasoning. \citet{perez-etal-2023-discovering, sharmatowards} identify "sycophancy", the tendency to align with user beliefs, as a pervasive failure mode. \citet{doshi2024generative} show that generative AI can reduce collective content diversity, potentially creating "echo chambers" \citep{jin2024agentreview, Hao2026} or navigating the "jagged technological frontier" unevenly \citep{dell2023navigating}.

Our collaborative architecture is motivated by theories of argumentation and Human-AI synergy \citep{Zhao_Liu_Wan_Tang_Li_2025, shao2025sciscigpt}. Evaluating scientific claims requires moving beyond semantic similarity \citep{reimers-2019-sentence-bert} to structural analysis \citep{Faigley-Witte-1981, yang-etal-2017-identifying-semantic}. To this end, our \assistant featured a revision-review module that analyzes a report’s argumentative structure using the schema proposed by \citet{toulmin1958}, alongside other linguistic frameworks \citep{teufel-moens-2002-articles, Mann1988RhetoricalST}. By evaluating how evidence supports specific statements in a consistent way across the full report and multiple authors' contributions, the \assistant was praised by the scientists for improving both the presentation and logical consistency of the output. AI shines in these linguistic tasks, which can be tedious and error-prone for humans, because they are largely mechanistic and are solely based on the input text, thus minimizing the risk of hallucinations.

Furthermore, historical analyses of Wikipedia \citep{Viegas-et-al-2004, Kittur-Kraut-2008} suggest that high-quality synthesis can emerge from complex dynamics \citep{yasseri2012dynamics} and reputation mechanisms \citep{Adler-Alfaro-2007}. We position the AI not as an oracle, but as a facilitator of collective deliberation \citep{tessler2024ai, summerfield2025impact, duenez2025perceptual}. This aligns with the vision of an AI co-scientist evaluated via rigorous methodologies \citep{cappello2025eaira}.

==> sections/2-ai-assistance.tex <==
\section{The AI Environment}
\label{sect:ai-assistance}

\begin{table*}[ht]
    \centering
    \caption{\small Summary of: lengths of input/output (Length), number of references (References), unique contributing authors (Authors), number of versions excluding the AI draft (Versions) and elapsed time (Time, hours:minutes format). Length is measured in number of words. Length and number of references are given for the draft proposed by Gemini (In), and for the final version curated by the scientists (Out).}
    \label{tab:top-metrics}
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{clccccccc}\toprule
        \multirow{2}{*}{\textbf{Phase}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Document}}} & \multicolumn{2}{c}{\textbf{Length}} & \multicolumn{2}{c}{\textbf{References}} & \multirow{2}{*}{\textbf{Authors}} & \multirow{2}{*}{\textbf{Versions}} & {\textbf{Time}}\\
         \cmidrule(lr){3-4} \cmidrule(lr){5-6}
          & & {\bf In} & {\bf Out} & {\bf In} & {\bf Out} & & & \textbf{(h:m)} \\\midrule
         {\bf1} & Outline   & 798 & 2107 & 0 & 0 & 8 & 16 & 05:17\\ \cmidrule{1-9}
         \multirow{6}{*}{{\bf2}} & 1. Introduction & 501 & 526 & 5 & 6 & 1 & 2 & 00:30 \\
          & 2. The Physical Science Basis of AMOC & 410 & 1400 & 3 & 14 & 3 & 9 & 03:30 \\
          & 3. Evidence for Variability and Slowdown & 675 & 2376 & 7 & 31 & 4 & 30 & 14:48 \\
          & 4. The Tipping Points Debate & 606 & 1662 & 3 & 13 & 4 & 12 & 04:28 \\
          & 5. Impacts, Risks and Vulnerabilities & 785 & 1345 & 7 & 13 & 6 & 20 & 09:47 \\
          & 6. Conclusion and Priorities & 498 & 960 & 7 & 18 & 3 & 5 & 00:45\\\cmidrule{2-9}
          & Total Phase 2      & 3475 & 8269 & 26 & 79 & 13 & 78 & 33:50\\\cmidrule{1-9}
         {\bf3} & Full Report & 7787 & 7918 & 79 & 67 & 4 & 10 & 07:28 \\\cmidrule{1-9}
         {\bf All} & Outline+Sections+Full Report & 798 & 7918 & 0 & 67 & 13 & 104 & 46:36\\\bottomrule
    \end{tabular}
\end{table*}
To isolate the impact of the collaborative workflow, we utilize a standard architecture consisting of three main components (see Figure~\ref{fig:editor-screenshot} in the Appendix for a screenshot). We use Gemini, as the LLM, accessed through \href{https://cloud.google.com/vertex-ai}{Vertex AI}.

\subsection{Editor}
An \emph{editor panel} provides a minimal text editor which accepts Markdown inputs for document formatting, and the inclusion of URLs for references. Edit actions can be manual or executed by AI. Edit instructions for AI are entered as document-level, or text span-level, feedback. The latter is triggered by text highlighting (cf. Figure~\ref{fig:editor-screenshot}). The same feedback mechanism (document or text span based) can be used to send messages to the human co-authors or inquire about the edit history of the relevant content.

\subsection{Evidence}
An \emph{evidence panel} provides a list of documents, that are used in the LLM's context.
Entries include a generated summary snippet, bibliographic information (title, authors, venue) and metadata (e.g., citations) retrieved from \href{https://openalex.org}{OpenAlex}. 

For a document to be used as a reference, authors need to add it to the evidence panel first, either by direct upload or via a built-in search function. 
In addition to results from Google Search, we also implement lookup from a collection of around 1,660 scientific papers on the topic of AMOC, that were collected and retrieved in advance. For this corpus we convert papers to Markdown using the LLM and use both BM25~\citep{bm25} and dense retrieval~\citep{karpukhin-etal-2020-dense} on document chunks. See Appendix \ref{sec:rag-settings} for implementation details.

\subsection{Assistant Chatbox}
A common \emph{chatbox} is available to ask questions to the \assistant. The LLM is rendered 'context-aware' by including in the input a representation of the \assistant \emph{state}: document, references, chat history etc. AI provides assistance in various other forms. When a user logs in, the \assistant provides a welcome message with a summary of the changes and discussion since the previous login (cf. Figure~\ref{fig:editor-screenshot}). The \assistant generates on demand a review of a revision, before submission, suggesting ways of improving the text based on rhetorical~\citep{Mann1988RhetoricalST,teufel-moens-2002-articles} and argumentative logic analysis~\citep{toulmin1958} of the updated report. The \assistant also helps resolving conflicts, proposing merges of concurrent revision candidates, as in code review workflows and version control systems.

\section{Assessment Workflow} 
The experiment was designed to approximate key features of IPCC-like assessments, including phased scoping, drafting, and iterative revision under explicit time constraints. The experiment took place over 5 weeks between November and December 2025. It involved a deliberately heterogeneous group of 13 climate scientists, spanning diverse sub-fields, with extensive experience as leads on IPCC and other institutional reports, and with varying levels of prior expertise on the Atlantic Meridional Overturning Circulation (AMOC), only a minority of whom had previously published directly on the topic. 
The process was executed in three \emph{phases}. Table~\ref{tab:top-metrics} reports high-level statistics about the process.

\paragraph{Phase 1 (Outline):} The \assistant generated an outline for a 10-page scientific assessment on AMOC's stability. Afterwards, the scientists edited the draft to produce the final outline and assigned themselves to specific sections. In Phase 1, we used Gemini 2.5 Pro as the LLM. Figure~\ref{fig:history-flow-outline} plots the history flow for the outline development.

\paragraph{Phase 2 (Sections):} Before Phase 2 we transitioned to the newly released Gemini 3 Pro Preview, due to its superior performance across multiple benchmarks. The expert-curated outline from Phase 1 was expanded by the \assistant into a full-length report draft, then segmented into sections. Each section was grounded in the AMOC corpus with a pipeline that evaluated all documents from the corpus, iteratively in batches. In each iteration, the \assistant identified the most relevant sources, replacing previous selections if more relevant ones were found. Finally, the \assistant revised the section text to incorporate in-text citations and references. The scientists then took over the drafts to curate, in groups, each individual section of the report. 



\paragraph{Phase 3 (Final Report):} In the last stage, the \assistant produced a new draft for the complete report by collating the different sections and producing a single coherent list of references and citations. A subset of the scientists then performed a final pass to improve the presentation, resolve any outstanding issues, check and sign off the content. As the very last step the \assistant performed an automatic reference check.



==> sections/3-results.tex <==
\section{Results}
\label{sect:results}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{images/convergence_plot_inverse.pdf}
    \caption{\small Document similarity scores over successive versions of the AMOC report, compared to the final version or step-wise.}
    \label{fig:convergence}
\end{figure}


\subsection{Convergence}
We expect that an effective consensus-based process will lead to an asymptotic convergence toward the final version of the document. We evaluate this hypothesis by computing text similarity metrics for each version. Specifically, we generate document embeddings\footnote{We use \texttt{\href{https://ai.google.dev/gemini-api/docs/embeddings}{gemini-embedding-001}} with task type \texttt{SEMANTIC\_SIMILARITY}} and calculate the inverse of the euclidean distance between each intermediate version and the final report.\footnote{Cosine similarity produces the same pattern but values are contained within a smaller interval near 1.0.}
We also compute the similarity between contiguous (step-wise) versions.

Figure~\ref{fig:convergence} illustrates the results. As anticipated, similarity to the final report converges almost monotonically. Three distinct stages emerge: 1) The process begins at a high baseline of similarity because the starting point is of high quality. During the first 9 versions, the report undergoes rapid changes. 2) The report enters a refinement stage characterized by smaller local changes. 3) A final stage begins with the transition to the pre-final version. A period of fine-tuning then follows until completion. Three roughly similar stages are also visible in the history flow plot of Figure~\ref{fig:history-flow-phases12-anonym}, in that case as a function of the document length.

\subsection{Efficiency}
Table~\ref{tab:top-metrics} reports logged-in \emph{elapsed time} for the sessions where the authors engaged in any one of the three phases. This metric should be interpreted as an approximation of time spent on the task rather than a precise measure of active work time. While we apply a timeout parameter (900 seconds) we may sometime underestimate idle time.  
Conversely, some activities outside of the tool, like offline proofreading, may not be accounted for. 

In this way, approximated total time spent writing and curating the report in the assistant is 46 hours, 36 minutes: $15\%$ of the time on Phase 1, $69\%$ on Phase 2 and $13\%$ on Phase 3, approximately 3.5 hours per author on average. 
As a first approximation, we guess an approximate speedup factor of 10x from four independent scientists' self-reported estimates. These range from 3–5x based on sub-tasks acceleration (writing, literature review), to 11–17x when extrapolating for full-time resource allocation and the reduction of collaborative communication overhead.
We emphasize that the \assistant is a prototype. It provides experimental features but it is unpolished and sometimes brittle. The authors spent some effort familiarizing themselves with the tool and were occasionally slowed down by bugs. Response latency was often noticeable, due to very long inputs and outputs. We cannot precisely quantify the time overhead due to learning and adaptation. A more polished tool would likely further improve efficiency. 

During the experiment, the 13 authors, in various configurations, iterated over 104 versions.\footnote{In Phase 2, 6 threads are developed in parallel, one per section. When combined in a single version history, they form 29 full versions of the report from Phase 2. Including the 10 versions from Phase 3 (and excluding the outline), the total is 39 report versions (cf. Figure~\ref{fig:history-flow-phases12-anonym} and Figure~\ref{fig:convergence}).} The outline length almost tripled in Phase 1, while the report sections length doubled in Phase 2, and marginally increased in the final pass. The number of references grew from 27, in the AI-generated draft of Phase 2, to 79 at the end of Phase 2, and finally to 67 at the end of Phase 3.  
Overall, the process involved substantial interventions on the text, and was thus highly efficient.

\subsection{Types of Interaction with AI}
\begin{table*}[t]
    \centering
    \caption{\small Types of interactions, and their counts, in the assistant in Phase 1 (Outline), Phase 2 (Sections) and Phase 3 (Full Report). 'Doc' means feedback relevant to the full report, while 'Span' means related to a specific span of text. }
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{llrrrrrrrrr}
    \toprule
    & & & \multicolumn{6}{c}{\bf Phase 2} & & \\
    \cmidrule(lr){4-9} 
    \multicolumn{2}{c}{{\bf Interaction}} & {\bf Phase 1} & {\bf \S1} & {\bf \S2} & {\bf \S3} & {\bf \S4} & {\bf \S5} & {\bf \S6} & {\bf Phase 3} & {\bf Total}\\ \midrule
\multirow{2}{*}{{\bf Revisions}} 
    & Manual & 11 & 0 & 1  & 31 & 5  & 14 & 0 & 0  & 62 \\
    & AI     & 32 & 3 & 20 & 78 & 29 & 50 & 8 & 25 & 245 \\ 
    \addlinespace[0.3em]
\multirow{2}{*}{\hspace{1em}\textit{of which submitted versions}}
     & Manual & 4  & 0 & 1 & 12 & 3 & 6  & 0 & 0  & 26 \\
     & AI     & 12 & 2 & 8 & 18 & 9 & 14 & 5 & 10 & 78 \\ \midrule
        \multirow{4}{*}{{\bf Feedback (to)}} 
            & AI (Doc)    & 2  & 0 & 4  & 2  & 8  & 5  & 0  & 4   & 25 \\
            & AI (Span)   & 45 & 8 & 20 & 80 & 38 & 68 & 10 & 116 & 385 \\
            & Human (Doc) & 1  & 0 & 0  & 4  & 1  & 0  & 0  & 0   &  6   \\
            & Human (Span)& 27 & 0 & 4  & 40 & 6  & 25 & 0  & 3   & 105 \\ \midrule
        \multirow{3}{*}{{\bf Tools}}     
            & Add Evidence& 0  & 1 & 0  & 0  & 0  & 2  & 0 & 0  & 3 \\
            & Search      & 9  & 0 & 10 & 24 & 2  & 9  & 4 & 2  & 60 \\
            & Chat        & 29 & 3 & 24 & 99 & 31 & 48 & 7 & 19 & 260 \\ \bottomrule
    \end{tabular}
    \label{tab:action-by-section}
\end{table*}

During a session, authors do not just revise the text. They search for evidence sources, chat with the \assistant to research topics, send messages to co-authors, ask the \assistant to revise the report and more.
Table~\ref{tab:action-by-section} reports statistics about the interactions types observed in the \assistant. There were 1,160 interactions in total (one every ~2.5 minutes on average), which we divide into three main categories: 

\noindent\textbf{Revisions:} By revision we mean any change to the document content, either via human edit (Manual) or via instructions to the Assistant (AI). Typically a session is characterized by multiple revisions, one of which is checked in as a new submitted version.

\noindent\textbf{Feedback:} Document-level (Doc) or text span-level (Span) feedback, either directed to AI or to the human co-authors.

\noindent\textbf{Tools:} Using the assistant tools to directly add articles (Add Evidence), search the corpus and the Web (Search) or chat with the assistant for various purposes (Chat).


\begin{table}[t]
    \centering
    \caption{\small Distribution of Chat Topics: Chats concern scientific topics and literature questions, cover the writing process, tool functionalities and tracing the history of specific passages.}
    \small
    \label{tab:requests}
    \begin{tabular}{lr}
        \toprule
        \textbf{Chat Topic} & \textbf{\%} \\
        \midrule
        Review and Critique & 28.4 \\
        Request Content Revision & 24.7 \\
        Manage Sources & 16.0 \\
        Get Help with the Tool & 11.5 \\
        Ask for Information &  11.5 \\
        Retrieve Change History & 7.8 \\        
        \bottomrule
    \end{tabular}
    \vspace{-.5em} 
\end{table}

About a third of the interactions involved feedback to the assistant on specific text spans - as instructions to generate revisions. The second most frequent interaction ($22.5\%$) are requests to the model to generate a new revision; model-generated revisions ($80\%$ of revisions, $75\%$ of submitted versions) are by far preferred over manual ones.
Authors engage frequently with the \assistant in chats ($21.7\%$ of interactions) and send messages to other authors ($9\%$ of interactions). 
Authors used the \assistant functionalities to search the document corpus (60 times) and to add sources manually by uploading individual papers (3 times).


Table~\ref{tab:requests} summarizes the topics of the chats, as categorized by Gemini, showing that chats with the assistant cover a wide set of issues. Table~\ref{tab:chat-examples} provides examples of the different types of messages in the \assistant's chatbox.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \caption{\small Comparison of human-directed vs AI-directed feedback.}
    \label{tab:feedback-targets}
    \begin{tabular}{lrr}
        \toprule
        \textbf{Feedback type} & \textbf{AI-directed} & \textbf{Human-directed} \\
        \midrule
        Epistemological & 56\%  & 42\% \\
        Presentation    & 22\%  & 48\% \\
        Sources         & 17\%  & 8\% \\
        Tone            & 5\%   & 2\% \\
        \bottomrule
    \end{tabular}
\end{table}

Table~\ref{tab:feedback-targets}  categorizes feedback distinguishing between \emph{epistemological} matters -- dimensions such as accuracy, specificity, completeness and uncertainty, \emph{evidence} (sources), \emph{presentation} and \emph{tone}~\citep{bulian2024}. Feedback directed to AI differs somewhat from the human-directed feedback. The majority of the feedback to AI involves knowledge quality (epistemological) issues, while the human-directed feedback concerns presentation and knowledge. Table~\ref{tab:feedback-examples} provides examples of feedback to AI for the different categories, Table~\ref{tab:messages-examples} provides examples of messages to co-authors.

\subsection{AI's Contribution to Revisions Content}
\begin{table}[ht]
\centering
\footnotesize
\setlength{\tabcolsep}{1pt}
\caption{\small Revision attribution: Estimated percentage of the content of AI-generated versions which is credited to AI. The Revision row reports counts.}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l rrrrrrrr @{}} 
\toprule
                   & Outline & \S1  & \S2  & \S3  & \S4  & \S5  & \S6  & Report \\ 
\midrule
\textbf{Revisions} & 16      & 2    & 9    & 30   & 12   & 20   & 5    & 10 \\
%\textbf{Human}     & 62      & 100  & 71   & 69   & 84   & 75   & 96   & 87 \\
\textbf{AI (\%)}        & 38      & 0    & 29   & 31   & 16   & 25   & 4    & 13 \\ 
\bottomrule
\end{tabular}
\label{tab:revision-attribution}
\end{table}

Scientists edit the text directly, or provide critical \emph{feedback} and \emph{instructions} for the \assistant to revise the text. The AI-proposed revision, in turn, is accepted or rejected by the human, further worked on etc. 
Table~\ref{tab:revision-attribution} summarizes the results of an estimate (based on Gemini) of the fraction of revisions that can be attributed to AI vs Human. For example, an instruction such as "Are there more bullet points to add on Mitigation?" would lead to some credit to AI, if the AI made some suggestions and the revision was checked in. Similarly, sometimes the model 'overgenerates', editing more than required. If the proposal is accepted this leads to some credit for the \assistant. The weighted average of the AI-credited revision content is $25.4\%$ (cf. \S\ref{sec:attribution-example} for an example).

At the same time, the \assistant can struggle to follow instructions. We observed a few errors in synthesizing number ranges from different sources (e.g., with respect to temperatures cooling in response to AMOC collapse); in these cases AI may pick a single number, from a single source. When requested to use specific criteria to make robust comparisons the model output was not always convincing. If pushed, adversarially, to take into account a study providing conflicting results AI may give the study a disproportional amount of space compared to the evidence from numerous other studies. This is a case of obsequious behavior, a well-known challenge for LLMs ~\citep{perez-etal-2023-discovering, sharmatowards}, which expert-in-the-loop frameworks may help improve upon.
Lack of comprehensiveness was also noted, e.g., in assessing types of impacts and response options.


\subsection{AI Contribution Metrics}
To evaluate the \assistant's contribution, we analyze the outline and report versions at the sentence level, using sentences as proxies for thematic units. We define a set of metrics that adapt ideas from well-established, reference-based, evaluation metrics for language prediction tasks such as machine translation, BLEU~\citep{papineni2002}, and summarization, ROUGE~\citep{lin-2004-rouge}.

Let $D$ be the set of sentences in the initial version proposed by the \assistant, the \emph{draft}. Let $F$ be the set of sentences in the \emph{final}, expert-curated version: the reference. We define an alignment $\mathcal{M}$ as a set of matching sentences:
\begin{equation}\nonumber \mathcal{M} = \{ (i, j) \mid \text{Sentence } D_i \text{ is aligned with } F_j \} \end{equation}
To account for many-to-many relationships (e.g., due to synthesis or expansion), we define alignments for both versions: 
\begin{align}\nonumber D_{\mathcal{M}} &= \{ i \in D \mid \exists j \in F : (i, j) \in \mathcal{M} \} \\ \nonumber F_{\mathcal{M}} &= \{ j \in F \mid \exists i \in D : (i, j) \in \mathcal{M} \} \end{align} 

\noindent\textbf{Precision (Retention)} \\ 
We use standard precision as a measure of \emph{thematic retention}: the amount of content proposed by AI that is still present in the expert-curated, version:
\begin{equation} \nonumber\text{Precision} = \frac{|D_{\mathcal{M}}|}{|D|} \end{equation} 
\textbf{Recall (Prevalence)} \\ Similarly, we use sentence recall as a measure of how \emph{prevalent} the AI content is in the ground truth version:
\begin{equation}\nonumber \text{Recall}= \frac{|F_{\mathcal{M}}|}{|F|} \end{equation}
Consequently, $1-\text{Recall}$ (the False Negative Rate) provides a measure of human contribution.

\noindent\textbf{F1 Score (Alignment)} \\ F1, the harmonic mean of Precision and Recall, summarizes the overall quality of the \emph{thematic alignment} from the perspective of both versions. \begin{equation}\nonumber F_1 = 2 \cdot \frac{\text{Precision} \cdot \text{Recall}}{\text{Precision} + \text{Recall}} \end{equation}

\begin{figure}
    \centering
%    \caption{Visualization of the results of the sentence alignment process for the AMOC report.}
    \includegraphics[width=1.0\linewidth]{images/alignment_asymmetric.pdf}
    \caption{Visualization of the results of the sentence alignment process for the AMOC report.}
    \label{fig:alignment}
\end{figure}
To compute the sentence alignment between versions, we used Gemini. This is a simple task for LLMs that can be solved effectively by leveraging self-attention, thus considering all possible cross-version and intra-version dependencies. We inspected all results manually and found them correct. Figure~\ref{fig:alignment} plots the output of the alignment process. The following example demonstrates how aligned (retained) content can be substantially expanded:

\noindent\textbf{Draft:} "3. Theory: Refine the theoretical application of Early Warning Signals to stochastic climate data to reduce false positives and negatives [24], [18]."

\noindent\textbf{Final:} "3. Theory: Move beyond purely statistical Early Warning Signals, which are prone to false positives [47], by developing and monitoring physics-based indicators, such as the freshwater transport at the southern boundary of the Atlantic [49], [66]."

Given that aligned content can vary semantically one should interpret the metrics proposed merely as a characterization of the thematic alignment between versions.

\subsection{AI Contribution Results}
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{2pt}
    \caption{\small AI Contribution Metrics: Precision (Thematic Retention), Recall (Thematic Prevalence) and F1 scores (Thematic Alignment).}
    \label{tab:scores}
    \begin{tabular}{l cc cc ccc} 
        \toprule
        & \multicolumn{2}{c}{\textbf{Sentences}} & \multicolumn{2}{c}{\textbf{Matches}} & \multicolumn{3}{c}{\textbf{Scores (\%)}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
        \textbf{Dataset} & \textbf{Draft} & \textbf{Final} & \textbf{Draft} & \textbf{Final} & \textbf{P} & \textbf{R} & \textbf{F1} \\ 
        \midrule
        \textbf{Outline} & 82  & 121 & 81  & 76  & 98.7 & 62.8 & 76.7 \\
        \textbf{Report}  & 131 & 288 & 123 & 120 & 93.8 & 41.6 & 57.7 \\
        \bottomrule
    \end{tabular}
\end{table}

We compute the AI Contribution metrics for the outline (Phase 1) and for the full report (Phase 2 + Phase 3). For the latter, we compare the \assistant version prepared at the beginning of Phase 2, against the very final version of the report produced in Phase 3. Table~\ref{tab:scores} reports the results. The four versions are copied in the Appendix, Outline: Draft (\ref{sect:outline:draft}), Final (\ref{sect:outline:final}); Report: Draft (\ref{sect:report-draft}), Final (\ref{sect:report-final}).

Precision is almost perfect for both outline and report, indicating that the AI content is of high quality. 
At the same time, as the Recall figures show, significant expert intervention is required to complete the final output in both cases. Particularly so for the report. Overall, AI performs better at generating the outline (F1: $76.7\%$) than the full report (F1: $57.7\%$). Although the switch from Gemini 2.5 to 3 introduces a potential confounding factor, it seems reasonable to assume that outline generation is a simpler task than full report writing, as the latter requires greater technical depth and synthesis.

From a qualitative point of view, while the draft is a solid high-level summary, the final version of the paper is a more rigorous, complete, evidence-based scientific assessment. Matching sentences in the final version sometimes replace generic, colloquial or emotive phrasing ("pivotal", "crucial", "essential" etc.) with neutral and technical descriptions ("contributes substantially").  
The edited sentences use a more nuanced language and articulate uncertainty more transparently and consistently. 

Human interventions involve also substantive accuracy issues; e.g., regarding the qualification of consensus. In a notable departure from the draft, involving the statement that "the scientific community has achieved consensus that the AMOC is weakening", primarily due to human activity, the experts removed the consensus claim and characterized the state of knowledge as complex and debated. The scientists incorporated findings from recent research that depict a much more nuanced and sometimes contradictory picture of AMOC's stability. For example, discussing evidence, missed by the \assistant draft, from air-sea heat flux and hydrographic data that suggest the circulation has remained more stable than previously thought. At another point the scientists lowered the confidence on purely anthropogenic attribution of the weakening of AMOC from "Medium Confidence" to "Low Confidence".
In these cases, human experts embraced complexity while the \assistant seemed to smooth over conflicts to present a unified narrative. Section~\ref{sect:example-sentences}, in the Appendix lists several examples. 

Finally, with respect to evidence, the increase in number of references was accompanied by a qualitative improvement in source selection and relevance. The final list of references includes foundational sources, and introduced a broader, more balanced, set of evidences as well as increasing the technical depth of the literature.


==> sections/4-discussion.tex <==
\section{Discussion}
There is a fundamental distinction between scientific review and assessment. A review is a summary of existing work, an overview of what the scientific literature says. While time-consuming it is technically straightforward. Advances in language modeling and retrieval suggest that literature review is an area of steady, iterative progress~\citep{delgado-chaves-2025}. The objective of the review process is sometimes called the “What”~\citep{Borton1970}.
Generative AI excels at this kind of general level summarization. 

A scientific assessment, instead, is a critical evaluation of quality, robustness, and uncertainty of the state of knowledge, and requires detailed understanding of the approaches, methods and theories underlying the available evidence (the "So What"). In the case of AMOC, much of this expertise is held by only a handful of specialists worldwide and may involve tacit knowledge (e.g. on model construction and internal testing) that is not publicly documented, thus not accessible to AI through peer-reviewed, or even gray literature. Our findings suggest that because AI cannot yet replicate this level of judgment, it is important to research frameworks where human experts  work alongside AI in a "human-in-the-loop" approach to learn to execute these complex analytical tasks, assisted by specific insights that go beyond what is publicly available. This may turn out to be a stepping stone toward the ability to identify research gaps, formulate implications, recommendations, and scientific discovery (the "Now What").

While AI can boost productivity, research suggests that it can narrow focus and hurt exploration~\citep{barrett2024,Hao2026}. Hybrid environments that facilitate the collaboration in large and diverse groups can help mitigate the risks of intellectual homogenization. In our experiment it is clear from the results that scientists did not merely edit the \assistant's work; they expanded and improved the \assistant's proposals, adding most of the final report’s content ($58\%$ human vs. $42\%$ AI). This indicates that the \assistant draft served as a starting point, but did not limit the assessment.


==> sections/5-conclusion.tex <==
\section{Conclusions}
In our experiment, 13 scientists completed a synthesis of 79 papers in 46 total person-hours to arrive at a scientific assessment of a complex topic. The work involved 104 revision cycles. AI-generated revisions were utilized 3 times more frequently than manual edits. Nearly 100\% of the AI-generated content was retained in the final report. Despite high retention, humans added 58\% of the final content ensuring technical depth and accuracy.

Our findings suggest that the scope of AI co-scientists can extend well beyond verification-rich tasks into open-ended research questions where ground truth and an authoritative state of knowledge is constructed through expert consensus. Hybrid intelligence architectures are central to this paradigm: while AI is highly effective at information processing, human expertise remains essential for ensuring scientific rigor, breadth, and nuance. This augmentative approach enables expert groups to accelerate research. Furthermore, embedding AI within expert workflows creates a feedback loop that may facilitate the acquisition of tacit process knowledge characteristic of advanced research, and the ability to integrate conflicting viewpoints. Moving forward, we envision these environments playing a central role in the development of trusted full-stack co-scientists. In the context of climate science, this paradigm may provide key tools to monitor and refine risk assessments of uncertain aspects of the climate system such as tipping points

\section*{Acknowledgments}
We thank Taylan Cemgil, Fernanda Viegas, Martin Wattenberg, Anna Koivuniemi, Ashley Thomas, Peter Battaglia, Ben Gaiarin and Elisa Rawat for feedback and support.

==> sections/amoc_final.tex <==
\newpage
\section*{AMOC Report: Final}
\label{sect:report-final}
\section*{An Assessment of Atlantic Meridional Overturning Circulation (AMOC) Stability: Tipping Points, Uncertainties, and Impacts}


\setcounter{subsection}{0}
The current scientific understanding of Atlantic Meridional Overturning Circulation (AMOC) stability. This assessment will encompass its physical science basis, associated risks, impacts, and vulnerabilities, and relevant mitigation or adaptation strategies, with a particular emphasis on conflicting evidence and scientific uncertainties surrounding potential tipping points and abrupt changes.

\subsection{Introduction}

\subsubsection{Definition and Importance of the AMOC}

The Atlantic Meridional Overturning Circulation (AMOC) is a system of ocean currents in the Atlantic Ocean (extending into the South Atlantic) characterized by a northward flow of warm, saline water in the upper layers of the Atlantic, and a southward flow of colder, deeper waters that are part of the thermohaline circulation [1]. While the AMOC utilizes the Gulf Stream as a pathway for its upper limb, it is important to distinguish the two; the Gulf Stream is primarily a wind-driven western boundary current, and both the wind-driven gyre and the overturning circulation contribute to the northward transport of heat [1].

This circulation system contributes substantially to Atlantic meridional heat transport, with estimates reaching up to ~1.3 PW at low to mid-latitudes [1], [2]. Beyond heat transport, the AMOC plays an important role in the global carbon cycle. Observational data indicate it facilitates the sequestration of anthropogenic carbon and heat in the deep ocean, thereby influencing the vertical and regional distribution of heat within the climate system [1], [3].

\subsubsection{The Emerging Concern: AMOC Instability and Abrupt Climate Change}
The stability of the AMOC has become a focal point of climate research due to its potential non-linear response to forcing [1], [4], [5]. Paleoclimate evidence and theory suggest that the AMOC may admit multiple stable regimes (strong and weak), with transitions possible under sufficient forcing [6]. Transitions between these states—such as those observed during Dansgaard-Oeschger (D-O) events or the Younger Dryas cooling—can occur rapidly on climatic timescales (decades to centuries) [5].

While past abrupt changes were often triggered by glacial meltwater pulses, modern concerns arise from anthropogenic climate change [2]. Accelerated melting of the Greenland Ice Sheet (GrIS), increased precipitation over the North Atlantic and enhanced freshwater fluxes from the Arctic are introducing growing amounts of freshwater into the North Atlantic [7]. This freshening reduces the density of surface waters, inhibiting the deep convection required to sustain the overturning circulation [7].

\subsubsection{Scope and Objectives}

This assessment aims to synthesize the state of knowledge regarding AMOC stability as of the publication date of the latest evidence included in this assessment. It specifically seeks to:
\begin{enumerate}
    \item Assess the physical mechanisms governing the circulation.
    \item Critically evaluate the tension between climate model projections (which generally show gradual weakening) and statistical Early Warning Signals (which suggest approaching tipping points).
   \item Assess the risks and vulnerabilities associated with AMOC decline.
\end{enumerate}

\subsection{The Physical Science Basis of AMOC}
\subsubsection*{Driving Mechanisms}
The AMOC is sustained by a complex interplay of buoyancy (thermohaline) and mechanical (wind-driven) forcing. While often conceptually framed as a ``push'' from high northern latitudes and a ``pull'' from the Southern Ocean, the circulation is largely in geostrophic balance and linked to basin-scale density gradients [8], [1].

\textbf{Buoyancy Forcing and Deep Water Formation (The ``Push''):} The density-driven component involves the formation of North Atlantic Deep Water (NADW). As warm, saline surface water flows northward, heat loss to the atmosphere cools it. This cooling, together with salinity increases from brine rejection during periods of extensive sea-ice formation, enhances water mass densification and can contribute to deep and intermediate water formation, particularly under glacial or near-glacial conditions [8].

\textbf{The Salt-Advection Feedback and Bistability:} The system's potential for bistability is closely linked to the salt-advection feedback. The Atlantic's narrow basin geometry, in combination with atmospheric moisture transport and basin-scale circulation, facilitates a salinity contrast distinct from the Pacific [9], which supports the transport of salt necessary for deep water formation. This positive feedback creates the potential for an abrupt transition to a collapsed 'off' state [10], [46]. However, this bistability is theoretically constrained by mechanical wind-driven forcing. If Southern Ocean wind forcing and mechanically driven upwelling play a dominant role in setting overturning strength and stability—a subject of active debate [8]—they may substantially modify the stability properties inferred from salt-advection-dominated models, reducing the likelihood or parameter range of multiple equilibria.

\textbf{Wind-Driven Forcing and Global Closure (The ``Pull''):} Closing the overturning circulation requires returning dense deep water to the surface. This upwelling is not merely a passive suction but is mechanically driven by two main processes: strong westerly winds in the Southern Ocean induce northward Ekman transport and divergence, effectively lifting deep waters (the Drake Passage effect), while wind- and tide-generated internal waves drive diapycnal mixing in the ocean interior [8].

\textbf{Variability Timescales:} Observations indicate that on shorter timescales (intra-annual), AMOC variability is often strongly influenced by local wind forcing, whereas on interannual to decadal timescales buoyancy forcing becomes increasingly important, with contributions that vary by latitude and AMOC metric [1].


\subsubsection*{Structure and Pathways}
The circulation is organized into two primary limbs, which constitute the Atlantic component of the global thermohaline circulation that transports heat, salt, and biogeochemical tracers:
\begin{itemize}
    \item \textbf{The Upper Limb:} This northward flow, which originates in the South Atlantic and feeds into the Gulf Stream and North Atlantic Current systems, transports warm, saline water in the upper approximately 1,000 meters [12]. Recent modeling indicates this limb also plays a vital role in transporting alkalinity and anthropogenic carbon to subpolar regions, which modulates the ocean's capacity for regional carbon uptake [13].
\item \textbf{The Lower Limb:} The southward return flow consists of cold, dense North Atlantic Deep Water (NADW), primarily traversing the Deep Western Boundary Current (DWBC) between 1,000 and 4,000 meters depth [12]. New observational evidence highlights the DWBC as an intense stream of bioavailable dissolved organic carbon (DOC), exporting it from the subpolar gyre to the deep subtropics where it fuels deep-ocean ecosystems [14].
\end{itemize}


\textbf{Deep Water Formation:} Understanding of deep water formation sites has been refined by recent observational arrays. While deep convection is vigorously active in the Labrador Sea, recent evidence from the OSNAP array suggests that the net transformation of light-to-dense water responsible for overturning occurs primarily in the eastern subpolar gyre (Irminger and Iceland basins) and the Nordic Seas [15]. Estimates of the AMOC's strength from the RAPID array at 26.5°N generally average around 17 Sv (Sverdup, $1Sv = 10^6 m^3s^{-1}$) [16], while recent hydrographic analyses over the last 90 years estimate the mean strength at approximately 18.4 ± 0.6 Sv [17].

\subsubsection*{AMOC’s Role in the Earth System}
The AMOC plays a fundamental role in regulating the Earth's climate through the redistribution of heat, carbon, and nutrients.

\begin{itemize}
    \item \textbf{Global Heat Redistribution:} The circulation transports significant heat northward. This meridional heat flux contributes substantially to maintaining the relatively mild climate of Northwestern Europe and regulating hemispheric heat balance [8], [1].
    \item \textbf{Carbon Sequestration and Ecosystem Support:} The AMOC acts as a critical pump for both inorganic and organic carbon, linking the surface and deep ocean:
    \begin{itemize}
    \item \textbf{Alkalinity and $CO_2$ Uptake:} The upper limb transports alkalinity northward, which enhances the North Atlantic's buffering capacity. This chemical transport is crucial for maintaining the region's ability to absorb anthropogenic $CO_2$ from the atmosphere [13].
    \item \textbf{Deep Ocean Fueling:} The sinking water masses export bioavailable dissolved organic carbon (DOC) via the Deep Western Boundary Current. This supply fuels deep-sea ecosystems, accounting for up to 38\% of the metabolic oxygen consumption in the deep North Atlantic [14]. 
    \end{itemize}
\item \textbf{ITCZ and Amazon Stability:} The inter-hemispheric energy imbalance created by the AMOC influences the position of the Intertropical Convergence Zone (ITCZ). Recent causal analysis suggests a stabilizing feedback loop: while a strong AMOC pulls the ITCZ northward, a weakening AMOC can shift rainfall patterns in a way that increases dry-season precipitation over the Southern Amazon, potentially offsetting drying trends in that critical biome [18].

\item \textbf{Decadal Variability:} A ``pacemaker region'' in the western transition zone between the subtropical and subpolar gyres has been identified as an important source region for decadal AMOC variability, which in turn influence sea surface temperature patterns that influence climate variability over surrounding landmasses [1].
\end{itemize}

\subsubsection*{Assessment of Evidence and Confidence}

There is \textbf{High Confidence} in the theoretical understanding of the component physical drivers of the AMOC (deep convection, geostrophic flow, and wind-driven transport) and its important role in global heat redistribution. While the general structural pathways are well-established, recent observations have refined the understanding of deep water formation sites, refining earlier views and highlighting the dominant role of the eastern subpolar gyre and Nordic Seas relative to the Labrador Sea [15]. There is increasing evidence supporting the AMOC's critical function in regulating regional carbon and alkalinity budgets [13], [14]. However, there remains \textbf{Medium Confidenc}e regarding the relative energetic contribution of buoyancy versus wind forcing in sustaining the overturning loop, as this remains an area of active research [8].

\subsection{Evidence for AMOC Variability: Past, Present, and Future}

Paleoclimatic Evidence of Past Abrupt Changes
The primary evidence that the AMOC is a bistable system—capable of existing in distinct ``on'' or ``off'' states—comes from the combination of paleoclimate evidence, theory, and modeling. Paleoclimatic records, including ice cores and marine sediments, are consistent with the AMOC crossing stability thresholds (tipping points) that trigger gradual or abrupt state transitions [19], [10]. These records extend our understanding beyond the short instrumental period and provide evidence of ocean-circulation changes during major climate reorganizations.

The Dansgaard–Oeschger events of the last glacial period illustrate the AMOC's capacity for rapid reorganization, featuring repeated, abrupt Northern Hemisphere warmings associated with circulation resurgences [20]. These events operated within a `climate see-saw' pattern, redistributing heat between hemispheres [20], and stood in sharp contrast to Heinrich stadials—periods of strongly reduced overturning driven by massive iceberg discharges and freshwater forcing [19]. This volatility continued through the last deglaciation, which unfolded as a sequence of abrupt transitions. Heinrich Stadial 1 (HS1; 18–14.7 ka) was a pronounced cold interval marked by high iceberg discharge and is widely viewed as a period of substantially reduced overturning [66]. This gave way to the Bølling–Allerød (14.7–12.6 ka), during which rapid North Atlantic warming coincided with a strong recovery of deep-water formation and a rapid reinvigoration of the AMOC, with broadly coherent climate responses across hemispheres as evidenced by multiple paleoceanographic proxies [21], [66].

The Younger Dryas event (approx. 12,900 years ago) serves as a potential analogue for a strongly weakened AMOC, although direct comparisons are limited by differences in boundary conditions (e.g., presence of the Laurentide Ice Sheet) [22]. Recovery from such collapsed states may involve rapid sea-ice feedbacks, such as the opening of polynyas, to restart deep water formation [22]. Modeling studies suggest that intermediate climate conditions may render the AMOC ``less stable'' than in peak glacial or interglacial conditions [66]. However, a long-standing ``meltwater paradox'' persists: most models require much larger freshwater fluxes to weaken the AMOC than those reconstructed from geological evidence of ice-sheet melting [23]. While most evidence for large AMOC reductions comes from glacial intervals, the 8.2 ka event in the early Holocene demonstrates that freshwater forcing can also weaken overturning during a warm interglacial climate, although the freshwater forcing during this event (catastrophic lake drainage) was likely larger than that expected in the near future [66][24].

\subsubsection*{Modern Observational Evidence}

\textbf{Opportunities and Challenges} 

Observing the AMOC involves balancing the accuracy of in-situ arrays with the spatial coverage of satellite data. In-situ arrays provide the gold standard for measuring volume transport but are spatially sparse, expensive, and offer records currently too short to robustly separate long-term anthropogenic trends from multi-decadal natural variability [25], [26]. Earth Observation (EO) technologies help bridge spatial gaps, though challenges remain in monitoring specific freshwater fluxes and transport variables [27], [28]. Moreover, current observational specifications generally do not satisfy the rigorous demands of tipping point early warning systems [28].

\textbf{Current State and Trends
}

Since 2004, the RAPID-MOCHA-WBTS array at 26.5°N has provided continuous, high-fidelity monitoring. This record reveals a weakening trend of approximately 1.0 Sv per decade over the 2004–2023 period [29]. Crucially, recent analysis of this record concludes that the observed weakening is consistent with climate model projections but ``not consistent with a collapse in the mid-21st century,'' providing robust observational evidence against a near-term collapse [29]. This decline, however, was not linear; it was most pronounced between 2004 and 2012, followed by a period of relative stability, though with high interannual variability strongly influenced by wind forcing [25], [30]. Additionally, the OSNAP array has highlighted that the majority of deep water transformation occurs in the eastern subpolar gyre, challenging earlier assumptions focused on the Labrador Sea [31]. Bridging the gap between sparse historical data and modern arrays, methods combining satellite altimetry with cable measurements have reconstructed variability back to 1993, aligning with the variability observed by arrays [32], [33].

\textbf{Indirect Proxies and Fingerprints
}

Due to the short duration of direct measurements, researchers rely on proxies. Reconstructions based on Sea Surface Temperature (SST), identifying the characteristic ``warming hole'' in the North Atlantic, suggest the AMOC has weakened by approximately 15\% since the mid-20th century and is in its weakest state in a millennium [34], [35]. However, surface signals can be contaminated by atmospheric ``noise'' [40]. Alternative reconstructions using subsurface density data, which capture deep circulation structure more directly, generally find no overall decline between 1981 and 2016, instead capturing a multi-decadal cycle [30]. Furthermore, hydrographic analyses extending back to the 1930s find no statistically significant decline in AMOC strength (estimating a decrease of only 0.4 ± 0.6 Sv with low confidence), which contradicts the significant weakening inferred from SST proxies [17].

New evidence challenges the robustness of SST-based proxies. Terhaar et al. (2025) show using 24 CMIP6 Earth System Models that subpolar SST anomalies ("warming holes") cannot robustly reconstruct the AMOC due to atmospheric noise and other factors. Instead, they propose that air-sea heat flux anomalies are a more physically robust proxy, tightly linked to AMOC strength through energy conservation on decadal timescales. Applying this method to ERA5 and JRA-55 reanalysis data, they reconstruct the AMOC at 26.5°N from 1963 to 2017 and find no decline, but rather substantial decadal variability [36]. This finding aligns with hydrographic evidence [17], [30] and clarifies that hydrographic data supports stability since the 1980s, but cannot address the mid-20th century decline directly inferred from SST.

To separate anthropogenic weakening from natural variability, recent analyses distinguish between a long-term ``Trend Mode,'' which exhibits the characteristic cooling pattern and a downward trajectory, and the Atlantic Multidecadal Oscillation (AMO) [37].

Beyond these spatial patterns, recent statistical analyses have identified signals consistent with critical slowing down in eight independent AMOC indices derived from observational SST and salinity data. These indices exhibit robust signs of critical slowing down (increasing variance and autocorrelation), suggesting a potential loss of stability over the last century [38].

\subsubsection*{Modeled Historical Evolution and Future Projections}

\textbf{Historical Evolution and Natural Variability:} Comparing observational proxies with climate models reveals discrepancies in the historical evolution of the AMOC. While SST-based fingerprints suggest a significant weakening since the mid-20th century [34], historical climate model simulations often depict a more stable circulation dominated by natural variability [39], [40]. For instance, analyses of CMIP6 historical simulations suggest that the multimodel mean AMOC strengthened from 1850 to 1985 due to anthropogenic aerosol forcing, contrasting with the weakening inferred from SST fingerprints [41]. Other studies argue that natural multidecadal variability has dominated since 1900, with models predicting only a minor slowing (approx. 1 Sv) after 1980 [39]. This divergence highlights uncertainties in separating forced signals from internal oscillations [42].


\textbf{Future Projections and Model Fidelity:} Despite historical discrepancies, CMIP6 models consistently project a weakening of the AMOC over the 21st century under all emission scenarios [54]. However, the magnitude varies significantly ($24\%$ to $39\%$ decline under high-emission scenarios). Standard resolution GCMs often suffer from biases, such as excessive stability due to poor representation of freshwater runoff spreading. Conversely, recent high-resolution models suggest resilience via eddy compensation mechanisms. However, recent studies using strongly eddying ocean-only models demonstrate that AMOC collapse is still possible under freshwater forcing, though eddies may maintain a weak ($~5 Sv$) residual circulation in the collapsed state [44].

\subsubsection*{Assessment of Evidence and Confidence}

While direct observations confirm a weakening trend in the early 21st century [25], there is \textbf{Low Confidence} in attributing a long-term decline solely to anthropogenic forcing relative to the pre-industrial era. This lower confidence reflects the growing divergence between SST-based proxies, which suggest a 15\% weakening [34], and a suite of alternative evidence including subsurface reconstructions [30], historical model simulations [39], hydrographic analyses [17], and physically-constrained heat flux inversions [36], all of which indicate stability or the dominance of natural variability since the mid-20th century. However, there is \textbf{Medium Confidence} that some indicators suggest a potential loss of stability (approaching a bifurcation point), evidenced by statistical early warning signals [38]. Furthermore, there is \textbf{High Confidence} that the AMOC has undergone rapid changes during the last glacial period and the deglaciation [6], [66].

\subsection{The Tipping Point Debate: Conflicting Evidence and Scientific Uncertainties}

The most contentious aspect of current AMOC science is the existence and proximity to a ``tipping point"—a critical threshold at which the system bifurcates from a strong mode (characterized by active overturning and heat transport) to a weak/off mode (where deep water formation is strongly reduced and circulation weakens substantially).

\subsubsection*{The Concept of Bistability and Hysteresis}

The potential for a tipping point arises from the non-linear dynamics of the salt-advection feedback. In the active ``on'' state, the AMOC transports salty water into the North Atlantic, maintaining the high surface density required for deep convection. A tipping point occurs when a perturbation—such as surface freshening or warming—weakens the circulation sufficiently that this salt transport is reduced, creating a self-amplifying feedback loop. If the salt transport drops below a critical threshold, the feedback reverses, preventing deep water formation and driving the system into a collapsed state [1], [46]. While this bistability implies hysteresis—meaning the pathway to recovery requires reducing forcing significantly below the collapse threshold—the core risk is the state shift triggered by the failure of the salt-advection pump [46].

\subsubsection*{Evidence Suggesting an Approaching Tipping Point}

Recent studies utilizing statistical physics have suggested an increased risk of a collapse within this century.

\begin{itemize}
    \item \textbf{Early Warning Signals (EWS):} As a complex system approaches a tipping point, it exhibits ``critical slowing down,'' characterized by increased variance and increased lag-1 autocorrelation in time-series data [45], [48]. Analyses of SST and salinity indices—including work by Boers (2021) and recent estimates by Ditlevsen \& Ditlevsen [38], [48]—suggest these signals may be present and statistically significant, with some studies estimating a potential collapse window within the 21st century [48].
\item \textbf{Dansgaard-Oeschger (DO) events:} Some general support, based on proxy data that a tipping of the AMOC might be detectable by prior EWS comes from DO events. DO events are characterized by millennial-scale abrupt climate changes during the glacial period, leading to abrupt temperature shifts in the North Atlantic region. Studies of climate bifurcation during the deglaciation suggest that such tipping points were approached in the past, providing qualitative support for the plausibility of EWS approaches [5].
\item \textbf{Overly Stable Models:} Physics-based indicators derived from observations suggest that many CMIP models are biased toward stability (the ``salt-advection feedback'' is modeled too weakly). Correcting for this bias suggests the real-world AMOC may be closer to a stability threshold than the model ensemble average indicates [45], [49].
\end{itemize}

\subsubsection*{Evidence Suggesting Greater Stability}
Contrasting the EWS studies, climate models generally project a more stable evolution.

\begin{itemize}

\item \textbf{Climate Model Projections:} The Coupled Model Intercomparison Project Phase 6 (CMIP6) models consistently project a weakening of the AMOC over the 21st century under all emission scenarios [45]. However, the magnitude varies significantly, with decline estimates ranging from 24\% to 39\% under high-emission scenarios. This consensus supports the assessment that while the AMOC will weaken, an abrupt collapse before 2100 is very unlikely (IPCC AR6 [50]).

\item \textbf{Observational Constraints:} Observations from the RAPID array suggest the recent weakening is consistent with climate models and not indicative of a collapse in the mid-21st century [29]. Furthermore, high-resolution models with realistic eddy fields often show low variability and a stable regime.

\item \textbf{High-Resolution Modeling:} Eddy-resolving models tend to show a more resilient circulation, suggesting that tipping behavior in some intermediate-complexity models may be sensitive to resolution [45].
\item \textbf{Stabilizing Feedback:} Mechanisms such as the warming of the deep ocean and changes in the gyre circulation may counteract the freshening signal.

\item \textbf{Critique of EWS:} Critics argue that EWS in climate data can be generated by changes in external forcing or ``red noise'' processes unrelated to bifurcation, leading to false positives [47]. Recent modeling by Zimmerman et al. [47] shows that Critical Slowing Down (CSD) indicators can robustly increase even in monostable regimes where no tipping point exists, suggesting these signals may not reliably distinguish between a slowing and a collapsing circulation.
\end{itemize}

\subsubsection*{Key Scientific Uncertainties}

The divergence in assessment stems from four deep uncertainties:

\textbf{Freshwater Hosing Plausibility and Model Bias}

A critical uncertainty is the magnitude of freshwater input required to trigger a collapse. There is a significant discrepancy between the stability of standard climate models and those corrected for known biases.

\begin{itemize}
    \item \textbf{Stability Bias: }Standard Global Circulation Models (GCMs) often exhibit a ``stability bias'' because they poorly represent the salt-advection feedback [45]. Consequently, these models often require extreme, potentially unrealistic freshwater ``hosing'' fluxes to induce a shutdown.
\item \textbf{Realistic Thresholds:} When corrected for this bias to match observed salinity budgets, the AMOC becomes significantly more sensitive. Research indicates that in bias-corrected models, the forcing generated by a doubling of $CO_2$ may be sufficient to trigger a collapse in some bias-corrected models, without the need for extreme external hosing [45], [49].
\end{itemize}

\textbf{Comparison of AMOC Stability Thresholds}

% \begin{table}[H]
%     \centering
\begin{center}
    \captionof{table}{Comparison of Model Stability}
    \label{tab:simple_comparison}
    \small % Slightly smaller font often helps with dense tables
    \begin{tabularx}{\textwidth}{lXXX}
        \toprule
        \textbf{Model Type} & \textbf{Stability Characteristics} & \textbf{Trigger for Collapse} & \textbf{Plausibility of Trigger} \\
        \midrule
        
        \textbf{Standard GCMs} & 
        High Stability: Salt-advection feedback is modeled too weakly [45]. & 
        Extreme Hosing: Requires large, artificial freshwater fluxes often exceeding realistic melt rates. & 
        Low: The required fluxes may be physically implausible under standard climate change scenarios. \\
        \addlinespace % Adds a tiny bit of breathing room between rows
        
        \textbf{Bias-Corrected} & 
        Realistic Sensitivity: Adjusted to match observed Atlantic salinity distribution [45, 49]. & 
        Climate Forcing: Can collapse under realistic warming scenarios (e.g., doubling of CO$_2$) due to internal hydrological changes. & 
        High: The trigger conditions fall within the range of expected future greenhouse gas forcing. \\
        
        \bottomrule
    \end{tabularx}
    \end{center}

% \end{table}

% Model Type
% Stability Characteristics
% Trigger for Collapse
% Plausibility of Trigger
% Standard GCMs
% High Stability: Salt-advection feedback is modeled too weakly [45].
% Extreme Hosing: Requires large, artificial freshwater fluxes often exceeding realistic melt rates.
% Low: The required fluxes may be physically implausible under standard climate change scenarios.
% Bias-Corrected Models
% Realistic Sensitivity: Adjusted to match observed Atlantic salinity distribution [45], [49].
% Climate Forcing: Can collapse under realistic warming scenarios (e.g., doubling of CO₂) due to internal hydrological changes.
% High: The trigger conditions fall within the range of expected future greenhouse gas forcing.

\textbf{Model Fidelity and Biases
}

Standard resolution GCMs often suffer from biases, such as the inability to resolve overflow processes and mesoscale eddies accurately [45]. Conversely, recent high-resolution models that resolve ocean eddies suggest the AMOC may be more stable, attributing this resilience to eddy compensation mechanisms [45]. However, recent studies using strongly eddying ocean-only models demonstrate that AMOC collapse is still possible under freshwater forcing, though eddies may maintain a weak (~5 Sv) residual circulation in the collapsed state [44]. This creates a divergence in the evidence base regarding the precise stability threshold and collapsed state characteristics.

\textbf{Signal vs. Noise
}

Distinguishing a trend toward a tipping point from natural multidecadal variability or forced response remains difficult [47]. While statistical analyses suggest an increased risk of collapse within this century [48], critics argue that these signals can be generated by ``red noise'' processes or changes in external forcing unrelated to bifurcation, raising concerns that these methods may yield false positives [47].

\textbf{Timing and Delays
}

Even if the AMOC tipping threshold is crossed, the timing of the subsequent collapse remains highly uncertain due to the ``slow passage effect.'' Kim et al. [52] demonstrate that under time-varying freshwater forcing, the system can exhibit a significant lag—potentially up to 1,300 years—between passing the bifurcation point and the actual circulation collapse. This implies that observation-based EWS might detect the threshold crossing long before the full climatic impacts fully manifest [52].


\subsubsection*{Assessment of Evidence and Confidence}

There is \textbf{Low Confidence} in the timing of a potential collapse. While the IPCC assessment remains the standard, the recent emergence of EWS studies based on statistical physics [48] and bias-corrected model analyses [49] suggests the risk is non-negligible and potentially underestimated [45]. There is \textbf{Medium Confidence} that the risk of crossing a tipping point increases non-linearly with cumulative emissions of greenhouse gases.

\subsection{Impacts, Risks, and Vulnerabilities of AMOC Decline}

The potential decline of the Atlantic Meridional Overturning Circulation (AMOC) poses systemic and severe risks to the climate system, ecosystems, and human societies. Assessing these risks requires distinguishing between the impacts of a gradual slowdown, which has been observed over parts of the instrumental period and is projected to continue in most models, and the profound global climate shifts that would result from an abrupt collapse. Such a collapse represents a critical transition or ``tipping point,'' which could occur if self-amplifying feedbacks, such as the salt-advection mechanism, become dominant [45].

\subsubsection*{Consequences of Gradual Weakening}

A gradual weakening of the AMOC alters heat distribution, sea-level patterns, and ocean biogeochemistry, creating a baseline of risk even without a full collapse.

\begin{itemize}
\item \textbf{Ocean Circulation and Biogeochemistry:} A declining AMOC disrupts broader ocean circulation patterns, leading to nutrient depletion in surface waters and reducing the efficiency of the biological carbon pump. These changes affect marine productivity and carbon storage [45].
\item \textbf{Regional Cooling and Hydroclimate Extremes:} While the AMOC transports heat northward, its decline leads to a ``bipolar seesaw'' pattern with cooling in the Northern Hemisphere and slight warming in the Southern Hemisphere. Simulations and paleoclimatic data indicate that the AMOC contributes substantially to maintaining air temperatures over the North Atlantic and Europe 5°C to 8°C warmer than they would be in its absence [45]. Consequently, a weakening or collapse would induce a significant cooling tendency, estimated to involve seasonal temperature drops of 5°C to 8°C in winter [2], [49], [45], which in a future warming climate would compete with the background greenhouse gas-induced warming, potentially leading to reduced warming rates or localized cooling depending on the emission scenario [45]. Additionally, recent weakening trends and the associated ``cold blob'' of sea surface temperatures in the North Atlantic have been linked to summer heatwaves and drought conditions in Europe [1], [41]. This connection arises as AMOC-driven SST anomalies influence atmospheric circulation patterns, such as the jet stream, thereby increasing the frequency of extreme weather events over surrounding landmasses [1].
\item \textbf{Dynamic Sea-Level Rise:} The weakening circulation disrupts the geostrophic balance of the Gulf Stream, causing water to pile up along the North American coast. Models project this could contribute an additional 15–20 cm of sea-level rise to the U.S. East Coast by 2100, significantly increasing the frequency and severity of coastal flooding [53].
\item \textbf{Marine Ecosystems:} The reduction in overturning circulation alters nutrient supply to the surface ocean, leading to declines in Total System Biomass (TSB). Ecosystem modeling suggests that on top of anthropogenic climate change, TSB decreases by roughly 2\% to 4\% due to AMOC weakening, with regional declines reaching up to 30\%, disproportionately affecting high trophic levels [54].
\end{itemize}

\subsubsection*{Consequences of Abrupt Collapse}

Crossing a tipping point into a collapsed AMOC state would result in rapid and potentially long-lasting global climate shifts.

\begin{itemize}
    \item \textbf{Severe Cooling:} In a collapse scenario, the cessation of northward heat transport would lead to drastic cooling across the Northern Hemisphere. This would radically alter habitability and energy demand in regions such as Scandinavia and Great Britain [45].
\item \textbf{Tropical Rainfall Shifts:} The resulting inter-hemispheric energy imbalance would tend to shift the Intertropical Convergence Zone (ITCZ) southward. This shift is projected to cause severe drying in the West African Monsoon and Indian Summer Monsoon regions, with rainfall reductions of approximately 29\% and 19\% respectively [55].
\item \textbf{Amazon Stabilization vs. Destabilization:} While some models suggest a southward ITCZ shift could increase dry-season precipitation over the Southern Amazon, potentially stabilizing the rainforest [18], broader assessments warn that AMOC collapse could interact with other tipping elements, increasing the risk of cascading destabilization in the Amazon and ice sheets [55], [56].
\end{itemize}

\subsubsection*{Key Risk Assessment}

The interaction of physical hazards with exposed and vulnerable systems creates specific key risks. The following risk assessment adopts a multi-criteria framework consistent with IPCC approaches, evaluating hazards, exposure, vulnerability, magnitude of impacts, and limits to adaptation for key AMOC-related risks.

\textbf{
Key Risk 1: Global Food Security via Monsoon Disruption
}
\begin{itemize}
   
 \item \textbf{Hazard \& Exposure:} An abrupt AMOC collapse shifts the thermal equator and the ITCZ southward. This shift strongly affects the West African Monsoon (WAM) and Indian Summer Monsoon (ISM), regions that support billions of people [55].
 \item \textbf{Vulnerability:} Agricultural systems in West Africa and India are highly sensitive to AMOC-driven shifts in the ITCZ due to their heavy dependence on rain-fed agriculture.
\item \textbf{Magnitude:} Multi-model comparisons indicate substantial disruptions, with ensemble mean annual rainfall changes of -29\% for WAM and -19\% for ISM [55]. In Northern Europe, severe cooling could render current arable farming practices unviable; modeling for Great Britain suggests an AMOC collapse could reduce the area of arable land from 32\% to 7\% due to climatic unsuitability [57].
 \item \textbf{Adaptation Limits:} While technological adaptations such as widespread irrigation could theoretically ameliorate some effects, the costs and water requirements may be prohibitive, as demonstrated in assessments for Great Britain [57].
\end{itemize}

\textbf{Key Risk 2: Systemic Economic Impact via Carbon Feedback
}
\begin{itemize}
 \item \textbf{Hazard:} A weakening AMOC reduces the ocean's capacity to uptake carbon. Simulations reveal an approximately linear relationship between AMOC strength and carbon uptake reductions, constituting a positive carbon cycle feedback [58].
 \item \textbf{Vulnerability:} the global economy is vulnerable to the accelerated warming resulting from higher atmospheric $CO_2$ concentrations.
 \item \textbf{Magnitude:} This ``AMOC carbon feedback'' could increase the Social Cost of Carbon (SCC) by roughly 1\%. When incorporated into integrated climate-economy models, this feedback leads to additional global economic damages estimated in the trillions of dollars [58].
\end{itemize}

\textbf{Key Risk 3: Cascading Earth System Interactions
}

\begin{itemize}
    \item \textbf{Hazard:} The AMOC acts as a mediator in the global network of tipping elements. Its collapse alters global heat distribution, potentially triggering cascading interactions across multiple tipping elements [56].
    \item \textbf{Vulnerability:} Major tipping elements, including the Greenland Ice Sheet, West Antarctic Ice Sheet, and Amazon rainforest, are sensitive to temperature and precipitation changes driven by the AMOC.
    \item \textbf{Magnitude:} Interactions tend to destabilize the network. While specific feedbacks like increased rainfall in the Southern Amazon might offer local stabilization [18], the broader risk involves global domino effects that could accelerate ice sheet loss and ecosystem transitions [56].
\end{itemize}

\textbf{Key Risk 4: Coastal Infrastructure and Communities via Sea-Level Rise
}
\begin{itemize}
    \item \textbf{Hazard \& Exposure:} The weakening of the AMOC disrupts the geostrophic balance of the Gulf Stream, causing water to pile up against the North American coast. This dynamic sea-level rise (DSL) acts on top of global mean sea-level rise [53].
    \item \textbf{Vulnerability:} Major population centers and infrastructure along the U.S. East Coast and the Gulf of Mexico are particularly vulnerable to this ``hotspot'' of sea-level rise [53].
    \item \textbf{Magnitude:} Modeling indicates that the anthropogenic signal in extreme sea levels can emerge quickly, with dynamic sea level contributing significantly to flood risk. For example, along the Northeast Coast, dynamic sea level rise is projected to reach up to ~20 cm by 2100 under high emission scenarios, significantly reducing the return period of extreme flooding events [53].
    \item \textbf{Adaptation Limits:} Response strategies involve a trade-off between hard protection (e.g., sea walls), which requires substantial public investment and engineering, and managed retreat, which entails significant social and economic costs for affected communities [67].
\end{itemize}

\subsection{Response Strategies}

Given the deep uncertainty regarding the proximity of an AMOC tipping point, strategies must prioritize resilience, robustness, and risk avoidance.

\textbf{Strategies for Gradual Weakening
}

\begin{itemize}
    \item \textbf{Adaptation to Gradual Change:} Strategies for gradual weakening focus on robust adaptation planning that avoids lock-ins while managing uncertainty [59]. In the agricultural sector, farmers and agribusinesses can implement robust adaptation planning, such as adjusting crop varieties; modeling indicates that under standard climate change scenarios involving gradual AMOC weakening, arable farming in regions like Great Britain remains largely viable with conventional adaptations [57]. Similarly, fisheries managers can implement sectoral adjustments, such as shifting quotas and targeting different species [54]. Conventional options also include coastal management agencies reinforcing coastal defenses against dynamic sea-level rise [53].
\end{itemize}
\textbf{
Strategies for a Potential Abrupt Collapse
}
\begin{itemize}
    \item \textbf{Transformational Adaptation:} A tipping point scenario necessitates transformative options beyond incremental adjustments. This includes national governments planning for radical shifts in land suitability, such as the potential cessation of arable farming in parts of Northern Europe [57].
\item \textbf{Emergency Contingencies:} Strategies involve developing contingencies for rapid climatic shifts that could overwhelm standard disaster risk management systems, particularly regarding food security in monsoon-dependent regions [55].
\end{itemize}

\textbf{Robust Strategies
}

\begin{itemize}
    \item\textbf{Flexible Adaptation Pathways:} To address deep uncertainty, policymakers should develop adaptation pathways that remain viable across a range of AMOC futures, from gradual weakening to collapse [59].
    \item\textbf{Scenario Broadening:} Assessments suggest broadening planning scenarios to include high-impact, low-probability events like AMOC collapse, ensuring that long-term infrastructure and policy decisions are robust to extreme outcomes [59].
    \item\textbf{Monitoring and Early Warning: }Continuous monitoring is crucial for detecting early warning signals (EWS). Recent statistical analyses have suggested the possibility of a collapse as early as mid-century [48], although these estimates remain controversial due to uncertainties in historical data and model assumptions [60].
    \item\textbf{Mitigation:} The most effective strategy to minimize the probability of crossing a tipping point is the rapid reduction of greenhouse gas emissions. Phasing out fossil fuels limits the freshwater forcing from ice melt that destabilizes the AMOC [45].
\end{itemize}


\subsection{Conclusion and Priorities for Research and Assessment}

\subsubsection*{Synthesis of Knowledge}

Multiple lines of observational and proxy evidence suggest that the AMOC may have weakened relative to the mid-20th century [45], [61]. However, this interpretation is challenged by hydrographic reconstructions [17], [30] and air-sea heat flux inferences [36] which suggest the circulation has remained stable over the last 30 to 90 years. Assessing these conflicting perspectives, while longer-term proxy records [61] suggest a weakening, recent reconstructions based on air-sea heat fluxes [36] and hydrographic data [17], [30] find no decline since the mid-20th century. This suggests that the ``warming hole'' signal used in earlier proxies may be less tightly coupled to AMOC strength than previously thought [36]. While recent research highlights the significant role of natural multidecadal variability in observed signals [39], ``fingerprint'' analyses and aerosol-forcing studies indicate that human activity is acting as a force multiplier on the system [45], [62]. Furthermore, a critical discrepancy exists regarding stability: while some high-resolution models depict a stable regime [51], [45], observation-based early warning signals suggest the system may be losing resilience [38]. Assessment of these conflicting lines of evidence suggests that models may currently underestimate the risk of abrupt change due to potential structural biases [63], [64].

In summary, it is \textbf{very likely} that the AMOC will weaken over the 21st century [50]. Furthermore, it is considered \textbf{very unlikely} that an abrupt collapse (tipping point) will occur before 2100 based on the current climate model ensemble consensus [50]. However, there is \textbf{Low Confidence} in the precise timing and magnitude of future changes given potential biases in current models [45], [49] and recent statistical Early Warning Signals (EWS) suggesting the system may be closer to a stability threshold than some models indicate.

\subsubsection*{Priorities for Strengthening Future Assessments}

\begin{itemize}
    \item \textbf{Observation:} Sustain and expand the RAPID and OSNAP arrays [12] with a specific focus on distinguishing long-term anthropogenic trends from multi-decadal natural variability [39]. Integrate these with Deep Argo and satellite gravimetry to reconstruct broader circulation patterns [65].
    \item \textbf{Modeling:} Investigate the structural causes of AMOC stability in climate models. While some high-resolution, eddy-resolving models suggest the system is more stable than previously thought [51], others indicate it remains vulnerable to freshwater forcing [63]. Resolving this discrepancy is urgent.
    \item \textbf{Theory:} Move beyond purely statistical Early Warning Signals, which are prone to false positives [47], by developing and monitoring physics-based indicators, such as the freshwater transport at the southern boundary of the Atlantic [49].
    \item \textbf{Impact Assessment:} Couple climate models simulating AMOC collapse with Integrated Assessment Models (IAMs) to quantify economic and social risks, particularly regarding the social cost of carbon [58].
\end{itemize}

\subsection{Final Remarks}

Although the precise attribution of recent weakening is complex and debated [39], [61], [30], the theoretical robustness of AMOC bistability [45], [64] supports the physical plausibility of abrupt collapse. Given the catastrophic global impacts of such an event, the inability of current models to rule out this risk necessitates a precautionary approach. Consequently, mitigation—the rapid reduction of greenhouse gas emissions—remains the only robust strategy to minimize the probability of crossing a potential tipping point [45].

\textbf{References:
}

[1] M. W. Buckley and J. Marshall, ``Observations, inferences, and mechanisms of the Atlantic Meridional Overturning Circulation: A review,'' Reviews of Geophysics, 2016. [Online]. Available: http://doi.org/10.1002/2015RG000493

%\bigskip

[2] W. Broeker, ``The great ocean conveyor,'' Oceanography, 1991. [Online]. Available: https://tos.org/oceanography/assets/docs/4-2\_broecker.pdf

%\bigskip

[3] V. Caínzos, A. Velo, F. F. Pérez, and A. Hernández‐Guerra, ``Anthropogenic Carbon Transport Variability in the Atlantic Ocean Over Three Decades,'' Global Biogeochemical Cycles, 2022. [Online]. Available: http://doi.org/10.1029/2022GB007475

%\bigskip

[4] J. van den Berk, S. Drijfhout, and W. Hazeleger, ``Characterisation of Atlantic meridional overturning hysteresis using Langevin dynamics,'' Earth System Dynamics, 2021. [Online]. Available: http://doi.org/10.5194/esd-12-69-2021

%\bigskip

[5] T. M. Lenton, V. Livina, V. Dakos, and M. Scheffer, ``Climate bifurcation during the last deglaciation?,'' Climate of the past, 2012. [Online]. Available: http://doi.org/10.5194/cp-8-1127-2012

%\bigskip

[6] S. Rahmstorf, ``Ocean circulation and climate during the past 120,000 years,'' Nature, 2002. [Online]. Available: https://www.nature.com/articles/nature01090

%\bigskip

[7] Q. Yang et al., ``Recent increases in Arctic freshwater flux affects Labrador Sea convection and Atlantic overturning circulation,'' Nature Communications, 2016. [Online]. Available: http://doi.org/10.1038/ncomms10525

%\bigskip

[8] T. Kuhlbrodt et al., ``On the driving processes of the Atlantic meridional overturning circulation,'' Reviews of Geophysics, 2007. [Online]. Available: http://doi.org/10.1029/2004RG000166

%\bigskip

[9] B. Sinha et al., ``Mountain ranges favour vigorous Atlantic meridional overturning,'' Geophysical Research Letters, 2011. [Online]. Available: https://doi.org/10.1029/2011gl050485

%\bigskip

[10] W. Weijer et al., ``Stability of the Atlantic Meridional Overturning Circulation: A Review and Synthesis,'' Journal of Geophysical Research Oceans, 2019. [Online]. Available: https://doi.org/10.1029/2019jc015083

%\bigskip

[11] H. Stommel, ``Thermohaline Convection with Two Stable Regimes of Flow,'' Tellus A Dynamic Meteorology and Oceanography, 1961. [Online]. Available: https://doi.org/10.1111/j.2153-3490.1961.tb00079.x

%\bigskip

[12] E. Frajka‐Williams, N. P. Foukal, and G. Danabasoglu, ``Should AMOC observations continue: how and why?,'' Philosophical Transactions of the Royal Society A Mathematical Physical and Engineering Sciences, 2023. [Online]. Available: http://doi.org/10.1098/rsta.2022.0195

%\bigskip

[13] Q. Zhang, T. Ito, and A. Bracco, ``Modulation of regional carbon uptake by AMOC and alkalinity changes in the subpolar North Atlantic under a warming climate,'' Frontiers in Marine Science, 2024. [Online]. Available: https://doi.org/10.3389/fmars.2024.1304193

%\bigskip

[14] M. Fontela, F. F. Pérez, H. Mercier, and P. Lherminier, ``North Atlantic Western Boundary Currents Are Intense Dissolved Organic Carbon Streams,'' Frontiers in Marine Science, 2020. [Online]. Available: https://doi.org/10.3389/fmars.2020.593757

%\bigskip

[15] T. Petit, M. S. Lozier, S. A. Josey, and S. A. Cunningham, ``Atlantic Deep Water Formation Occurs Primarily in the Iceland Basin and Irminger Sea by Local Buoyancy Forcing,'' Geophysical Research Letters, 2020. [Online]. Available: https://doi.org/10.1029/2020gl091028

%\bigskip

[16] W. E. Johns et al., ``Towards two decades of Atlantic Ocean mass and heat transports at 26.5° N,'' Philosophical Transactions of the Royal Society A Mathematical Physical and Engineering Sciences, 2023. [Online]. Available: https://doi.org/10.1098/rsta.2022.0188

%\bigskip

[17] T. Rossby, J. B. Palter, and K. Donohue, ``What Can Hydrography Between the New England Slope, Bermuda and Africa Tell us About the Strength of the AMOC Over the Last 90 years?,'' Geophysical Research Letters, 2022. [Online]. Available: https://doi.org/10.1029/2022gl099173

%\bigskip

[18] A. Högner et al., ``Causal pathway from AMOC to Southern Amazon rainforest indicates stabilising interaction between two climate tipping elements,'' Environmental Research Letters, 2025. [Online]. Available: http://doi.org/10.1088/1748-9326/addb62

%\bigskip

[19] A. H. L. Voelker and J. T. Andrews, ``Millennial-Scale Ocean Climate Variability,'' Encyclopedia of Ocean Sciences (Third Edition)", Academic Press, 2018. [Online]. Available: http://doi.org/10.1016/B978-0-12-409548-9.11368-5

%\bigskip

[20] North Greenland Ice Core Project members, ``High-resolution record of Northern Hemisphere climate extending into the last interglacial period,'' Nature, 2004. [Online]. Available: https://doi.org/10.1038/nature02805

%\bigskip

[21] T. Chen et al., ``Synchronous centennial abrupt events in the ocean and atmosphere during the last deglaciation,'' Science, 2015. [Online]. Available: https://doi.org/10.1126/science.aac6159

%\bigskip

[22] J. Velay‐Vitow, D. Chandan, and W. R. Peltier, ``Into the Holocene, anatomy of the Younger Dryas cold reversal and preboreal oscillation,'' Scientific Reports, 2024. [Online]. Available: http://doi.org/10.1038/s41598-024-53591-2

%\bigskip

[23] B. Snoll et al., ``A multi-model assessment of the early last deglaciation (PMIP4 LDv1): a meltwater perspective,'' Climate of the past, 2024. [Online]. Available: https://doi.org/10.5194/cp-20-789-2024

%\bigskip

[24] G. Rush et al., ``The magnitude and source of meltwater forcing of the 8.2 ka climate event constrained by relative sea-level data from eastern Scotland,'' Quaternary Science Advances, 2023. [Online]. Available: https://doi.org/10.1016/j.qsa.2023.100119

%\bigskip

[25] B. Moat et al., ``Pending recovery in the strength of the meridional overturning circulation at 26° N,'' Ocean science, 2020. [Online]. Available: http://doi.org/10.5194/os-16-863-2020

%\bigskip

[26] D. Lobelle et al., ``Detectability of an AMOC Decline in Current and Projected Climate Changes,'' Geophysical Research Letters, 2020. [Online]. Available: https://doi.org/10.1029/2020gl089974

%\bigskip

[27] R. Wood et al., ``Opportunities for Earth Observation to Inform Risk Management for Ocean Tipping Points,'' Surveys in Geophysics, 2024. [Online]. Available: https://doi.org/10.1007/s10712-024-09859-3

%\bigskip

[28] S. Loriani et al., ``Monitoring the Multiple Stages of Climate Tipping Systems from Space: Do the GCOS Essential Climate Variables Meet the Needs?,'' Surveys in Geophysics, 2025. [Online]. Available: https://doi.org/10.1007/s10712-024-09866-4

%\bigskip

[29] G. McCarthy et al., ``Signal and Noise in the Atlantic Meridional Overturning Circulation at 26°N,'' Geophysical Research Letters, 2025. [Online]. Available: https://doi.org/10.1029/2025gl115055

%\bigskip

[30] E. Worthington et al., ``A 30-year reconstruction of the Atlantic meridional overturning circulation shows no decline,'' Ocean science, 2021. [Online]. Available: https://doi.org/10.5194/os-17-285-2021

%\bigskip

[31] F. Li et al., ``Subpolar North Atlantic western boundary density anomalies and the Meridional Overturning Circulation,'' Nature Communications, 2021. [Online]. Available: http://doi.org/10.1038/s41467-021-23350-2

%\bigskip

[32] E. Frajka‐Williams, ``Estimating the Atlantic overturning at 26°N using satellite altimetry and cable measurements,'' Geophysical Research Letters, 2015. [Online]. Available: https://doi.org/10.1002/2015gl063220

%\bigskip

[33] A. Sanchez‐Franks, E. Frajka‐Williams, B. Moat, and D. Smeed, ``A dynamically based method for estimating the Atlantic meridional overturning circulation at 26° N from satellite altimetry,'' Ocean science, 2021. [Online]. Available: https://doi.org/10.5194/os-17-1321-2021

%\bigskip

[34] L. Caesar, S. Rahmstorf, A. Robinson, G. Feulner, and V. S. Saba, ``Observed fingerprint of a weakening Atlantic Ocean overturning circulation,'' Nature, 2018. [Online]. Available: http://doi.org/10.1038/s41586-018-0006-5

%\bigskip

[35] D. Thornalley et al., ``Anomalously weak Labrador Sea convection and Atlantic overturning during the past 150 years,'' Nature, 2018. [Online]. Available: https://doi.org/10.1038/s41586-018-0007-4

%\bigskip

[36] J. Terhaar, L. Vogt, and N. P. Foukal, ``Atlantic overturning inferred from air-sea heat fluxes indicates no decline since the 1960s,'' Nature Communications, 2025. [Online]. Available: https://doi.org/10.1038/s41467-024-55297-5

%\bigskip

[37] Dima, M., Lohmann, G., Ionita, M. et al., ``AMOC modes linked with distinct North Atlantic deep water formation sites,'' Clim Dyn, 2022. [Online]. Available: https://doi.org/10.1007/s00382-022-06156-w

%\bigskip

[38] N. Boers, ``Observation-based early-warning signals for a collapse of the Atlantic Meridional Overturning Circulation,'' Nature Climate Change, 2021. [Online]. Available: https://doi.org/10.1038/s41558-021-01097-4

%\bigskip

[39] M. Latif, J. Sun, M. Visbeck, and M. H. Bordbar, ``Natural variability has dominated Atlantic Meridional Overturning Circulation since 1900,'' Nature Climate Change, 2022. [Online]. Available: https://doi.org/10.1038/s41558-022-01342-4

%\bigskip

[40] G. D. McCarthy and L. Caesar, ``Can we trust projections of AMOC weakening based on climate models that cannot reproduce the past?,'' Philosophical Transactions of the Royal Society A Mathematical Physical and Engineering Sciences, 2023. [Online]. Available: https://doi.org/10.1098/rsta.2022.0193

%\bigskip

[41] M. Menary et al., ``Aerosol‐Forced AMOC Changes in CMIP6 Historical Simulations,'' Geophysical Research Letters, 2020. [Online]. Available: https://doi.org/10.1029/2020gl088166

%\bigskip

[42] J. Robson, R. Sutton, M. Menary, and M. W. K. Lai, ``Contrasting internally and externally generated Atlantic Multidecadal Variability and the role for AMOC in CMIP6 historical simulations,'' Philosophical Transactions of the Royal Society A Mathematical Physical and Engineering Sciences, 2023. [Online]. Available: https://doi.org/10.1098/rsta.2022.0194

%\bigskip

[43] Dima, M., Lohmann, G., Nichita, DR. et al., ``Structural stability changes of the Atlantic Meridional Overturning Circulation,'' npj Clim Atmos Sci, 2025. [Online]. Available: https://doi.org/10.1038/s41612-025-00960-x

%\bigskip

[44] R. M. van Westen, M. Kliphuis, and H. A. Dijkstra, ``Collapse of the Atlantic Meridional Overturning Circulation in a Strongly Eddying Ocean‐Only Model,'' Geophysical Research Letters, 2025. [Online]. Available: http://doi.org/10.1029/2024GL114532

%\bigskip

[45] S. Rahmstorf, ``Is the Atlantic Overturning Circulation Approaching a Tipping Point?,'' Oceanography, 2024. [Online]. Available: http://doi.org/10.5670/oceanog.2024.501

%\bigskip

[46] M. Hofmann and S. Rahmstorf, ``On the stability of the Atlantic meridional overturning circulation,'' Proceedings of the National Academy of Sciences, 2009. [Online]. Available: https://doi.org/10.1073/pnas.0909146106

%\bigskip

[47] C. Zimmerman, T. J. W. Wagner, E. Maroon, and D. E. McNamara, ``Slowed Response of Atlantic Meridional Overturning Circulation Not a Robust Signal of Collapse,'' Geophysical Research Letters, 2025. [Online]. Available: http://doi.org/10.1029/2024GL112415

%\bigskip

[48] P. Ditlevsen and S. Ditlevsen, ``Warning of a forthcoming collapse of the Atlantic meridional overturning circulation,'' Nature Communications, 2023. [Online]. Available: http://doi.org/10.1038/s41467-023-39810-w

%\bigskip

[49] R. M. van Westen, M. Kliphuis, and H. A. Dijkstra, ``Physics-based early warning signal shows that AMOC is on tipping course,'' Science Advances, 2024. [Online]. Available: https://doi.org/10.1126/sciadv.adk1189

%\bigskip

[50] Intergovernmental Panel on Climate Change, ``Climate Change 2021: The Physical Science Basis,'' Cambridge University Press eBooks, 2023. [Online]. Available: https://doi.org/10.1017/9781009157896

%\bigskip

[51] L. Gerber, J. Lippold, F. Süfke, O. Valk, P. Testorf, M. Ehnis, S. Tautenhahn, L. Max, C. M. Chiessi, M. Regelous, S. Szidat, O. Friedrich, F. Pöppelmeier, ``Low variability of the Atlantic Meridional Overturning Circulation throughout the Holocene.'' Nat Commun, 2025 [Online]. Available: https://pmc.ncbi.nlm.nih.gov/articles/PMC12284099/ 

%\bigskip

[52] S. Kim, H. Kim, H. A. Dijkstra, and S. An, ``Slow and soft passage through tipping point of the Atlantic Meridional Overturning Circulation in a changing climate,'' npj Climate and Atmospheric Science, 2022. [Online]. Available: https://doi.org/10.1038/s41612-022-00236-8

%\bigskip

[53] J. Yin, S. M. Griffies, M. Winton, M. Zhao, and L. Zanna, ``Response of Storm-Related Extreme Sea Level along the U.S. Atlantic Coast to Combined Weather and Climate Forcing,'' Journal of Climate, 2020. [Online]. Available: http://doi.org/10.1175/JCLI-D-19-0551.1

%\bigskip

[54] A. Boot, J. Steenbeek, M. Coll, A. S. von der Heydt, and H. A. Dijkstra, ``Global Marine Ecosystem Response to a Strong AMOC Weakening Under Low and High Future Emission Scenarios,'' Earth s Future, 2025. [Online]. Available: http://doi.org/10.1029/2024EF004741

%\bigskip

[55] M. Ben‐Yami et al., ``Impacts of AMOC Collapse on Monsoon Rainfall: A Multi‐Model Comparison,'' Earth s Future, 2024. [Online]. Available: http://doi.org/10.1029/2023EF003959

%\bigskip

[56] N. Wunderling, J. F. Donges, J. Kurths, and R. Winkelmann, ``Interacting tipping elements increase risk of climate domino effects under global warming,'' Earth System Dynamics, 2021. [Online]. Available: https://esd.copernicus.org/articles/12/601/2021/esd-12-601-2021.pdf

%\bigskip

[57] Smith, G. S., Ritchie, P.D.L., ``Modelled arable area for Great Britain under different climate and policy scenarios,'' NERC Environmental Data Service, 2019. [Online]. Available: http://doi.org/10.5285/e1c1dbcf-2f37-429b-af19-a730f98600f6

%\bigskip

[58] F. Schaumann and E. Alastrué de Asenjo, ``Weakening AMOC reduces ocean carbon uptake and increases the social cost of carbon,'' Proceedings of the National Academy of Sciences, 2025. [Online]. Available: http://doi.org/10.1073/pnas.2419543122

%\bigskip

[59] R. Biesbroek, M. Haasnoot, K. J. Mach, and A. C. Petersen, ``Adaptation planning in the context of a weakening and possibly collapsing Atlantic Meridional Overturning Circulation (AMOC),'' Regional Environmental Change, 2025. [Online]. Available: https://doi.org/10.1007/s10113-025-02434-5

%\bigskip

[60] M. Ben-Yami, A. Morr, S. Bathiany, N Boers, ``Uncertainties too large to predict tipping times of major Earth system components from historical data,'' Sci. Adv., 2024. [Online]. Available: https://doi.org/10.1126/sciadv.adl4841

%\bigskip

[61] L. Caesar, G. McCarthy, D. Thornalley, N. Cahill, and S. Rahmstorf, ``Current Atlantic Meridional Overturning Circulation weakest in last millennium,'' Nature Geoscience, 2021. [Online]. Available: https://doi.org/10.1038/s41561-021-00699-z

%\bigskip

[62] T. Hassan, R. J. Allen, W. Liu, and C. A. Randles, ``Anthropogenic aerosol forcing of the Atlantic meridional overturning circulation and the associated mechanisms in CMIP6 models,'' Atmospheric chemistry and physics, 2021. [Online]. Available: https://doi.org/10.5194/acp-21-5821-2021

%\bigskip

[63] D. Swingedouw et al., ``AMOC Recent and Future Trends: A Crucial Role for Oceanic Resolution and Greenland Melting?,'' Frontiers in Climate, 2022. [Online]. Available: http://doi.org/10.3389/fclim.2022.838310

%\bigskip

[64] E. Hawkins et al., ``Bistability of the Atlantic overturning circulation in a global climate model and links to ocean freshwater transport,'' Geophysical Research Letters, 2011. [Online]. Available: https://doi.org/10.1029/2011gl047208

%\bigskip

[65] H. Wei et al., ``Full‐Depth Reconstruction of Long‐Term Meridional Overturning Circulation Variability From Satellite‐Measurable Quantities via Machine Learning,'' Journal of Advances in Modeling Earth Systems, 2025. [Online]. Available: http://doi.org/10.1029/2024MS004915

%\bigskip

[66] S.K.V. Hines, , N.P. Foukal, K.M. Costa, D.W. Oppo, O. Marchal, L.D. Keigwin, and A. Condron. ``Is there robust evidence for freshwater-driven AMOC changes? A synthesis of data, models, and mechanisms.'' Oceanography 38(3), 2025.  [Online]. Available: https://doi.org/10.5670/oceanog.2025.e301

%\bigskip

[67] Glavovic, B.C., R. Dawson, W. Chow, M. Garschagen, M. Haasnoot, C. Singh, and A. Thomas, ``Cross-Chapter Paper 2: Cities and Settlements by the Sea.'' Climate Change 2022: Impacts, Adaptation and Vulnerability. Contribution of Working Group II to the Sixth Assessment Report of the Intergovernmental Panel on Climate Change, 2022, Available: https://doi.org/10.1017/9781009325844.019

%\bigskip

